Principal Component Analysis of Molecular Clouds: Can CO reveal the dynamics?

We use Principal Component Analysis (PCA) to study the gas dynamics in numerical simulations of typical MCs. Our simulations account for the non-isothermal nature of the gas and include a simplified treatment of the time-dependent gas chemistry. We model the CO line emission in a post-processing step using a 3D radiative transfer code. We consider mean number densities n_0 = 30, 100, 300 cm^{-3} that span the range of values typical for MCs in the solar neighbourhood and investigate the slope \alpha_{PCA} of the pseudo structure function computed by PCA for several components: the total density, H2 density, 12CO density, 12CO J = 1 -> 0 intensity and 13CO J = 1 -> 0 intensity. We estimate power-law indices \alpha_{PCA} for different chemical species that range from 0.5 to 0.9, in good agreement with observations, and demonstrate that optical depth effects can influence the PCA. We show that when the PCA succeeds, the combination of chemical inhomogeneity and radiative transfer effects can influence the observed PCA slopes by as much as ~ +/- 0.1. The method can fail if the CO distribution is very intermittent, e.g. in low-density clouds where CO is confined to small fragments.

==> journals.tex <==
%% journal abbreviations (from aastex.cls)

\def\jnl@style#1{{\rmfamily#1}}%
\def\jref@jnl#1{{\jnl@style#1}}%

\newcommand\aj{\jref@jnl{AJ}}%
          % Astronomical Journal
\newcommand\araa{\jref@jnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\jref@jnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\jref@jnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\jref@jnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\jref@jnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\jref@jnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\jref@jnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\jref@jnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\jref@jnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\jref@jnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\jref@jnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\jrasc{\jref@jnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\jref@jnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\jref@jnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\pra{\jref@jnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\jref@jnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\jref@jnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\jref@jnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\jref@jnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\jref@jnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasp{\jref@jnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\jref@jnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\jref@jnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\skytel{\jref@jnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\jref@jnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\jref@jnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\jref@jnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\jref@jnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\jref@jnl{Nature}}%
          % Nature
\newcommand\iaucirc{\jref@jnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\jref@jnl{Astrophys.~Lett.}}%
          % Astrophysics Letters
\newcommand\apspr{\jref@jnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\jref@jnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\jref@jnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\jref@jnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\jref@jnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\jref@jnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\jref@jnl{J.~Geophys.~Res.}}%
          % Journal of Geophysics Research
\newcommand\jqsrt{\jref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\jref@jnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\jref@jnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\jref@jnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\jref@jnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\jref@jnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\jref@jnl{Proc.~SPIE}}%
          % Proceedings of the SPIE

